MEDLEY: Intent-based Recommendations to Support Dashboard Composition

Despite the ever-growing popularity of dashboards across a wide range of domains, their authoring still remains a tedious and complex process. Current tools offer considerable support for creating individual visualizations but provide limited support for discovering groups of visualizations that can be collectively useful for composing analytic dashboards. To address this problem, we present MEDLEY, a mixed-initiative interface that assists in dashboard composition by recommending dashboard collections (i.e., a logically grouped set of views and filtering widgets) that map to specific analytical intents. Users can specify dashboard intents (namely, measure analysis, change analysis, category analysis, or distribution analysis) explicitly through an input panel in the interface or implicitly by selecting data attributes and views of interest. The system recommends collections based on these analytic intents, and views and widgets can be selected to compose a variety of dashboards. MEDLEY also provides a lightweight direct manipulation interface to configure interactions between views in a dashboard. Based on a study with 13 participants performing both targeted and open-ended tasks, we discuss how MEDLEY's recommendations guide dashboard composition and facilitate different user workflows. Observations from the study identify potential directions for future work, including combining manual view specification with dashboard recommendations and designing natural language interfaces for dashboard authoring.

==> README <==
Created by Torsten Moeller (vis@cs.sfu.ca), April 6 2004
modified by Steven Bergner and Torsten Moeller, June 30 2006
modified by James Peltier and Torsten Moeller, March 28, 2007
modified by Bernhard Finkbeiner, July 5, 2010
modified by Tobias Isenberg, January 2016
modified by Filip Sadlo, March 2016
modified by Tobias Isenberg, July 2016

This distribution provides a document class for formatting papers according to the specifications for submission to conferences sponsored by the IEEE Visualization & Graphics Technical Committee (VGTC).

Conferences that use the 'journal' document option:
- IEEE Visualization Conference (VIS, incl. InfoVis, SciVis, VAST)
- IEEE Virtual Reality (VR)
- IEEE International Symposium on Mixed and Augmented Reality (ISMAR)

It contains 13 files/directories:

README          - this file
diamondrule.eps - abstract and body separator
diamondrule.pdf - its PDF version
vgtc.cls        - the VGTC class file, which should be placed, somewhere in the TeX search path (or in the local directory)
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
template.pdf    - an example proper pdf output in default journal mode
abbrv-doi*.bst  - four different versions to generate the bibliography including DOI output, with and without hyperref support, with and without narrow rendering of DOIs
makefile        - makefile including bibtex compilation and proper PDF generation
pictures/       - subdirectory with sample images, both in EPS and in direct pixel/vector format

Usage
=====

The template can be used as such (using the established LaTeX environments) by calling pdfLaTeX or LaTex. For Windows-based LaTeX installations you can use, for example, the environment provided by http://www.texniccenter.org/ along with MikTeX (http://miktex.org/). For Uinux-based installations, please use your favorite LaTeX distribution and editing environment or use the makefile following the instructions below.

Use of the Makefile
===================

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create a file called 'template.pdf'. Please make sure, that its layout is identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process manually.  Below are a list of available options that may be passed to make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)


==> sections/archive/design-goals-Feb21.tex <==
\section{Design Goals}
\vidya{making this its own section where we fold in the survey details to talk about how they informed the compilation of the set of goals for Medley}
We followed an iterative design process to develop \medley's interface and features.

Specifically, over a span of six weeks, we had multiple meetings with the four dashboard design experts mentioned in Section~\ref{} as well as three additional designers and product managers who were less versed in dashboard authoring.
During these meetings, we asked participants about their dashboard design process and also demonstrated working versions of \medley's prototype to gather feedback on system features and interface ideas.
Combining the feedback from these meetings with guidelines and findings from prior work on visualization recommendation systems (e.g.,~\cite{key2012vizdeck,wongsuphasawat2015voyager,crisan2021gevitrec,wu2021multivision}), mixed-initiative interfaces~\cite{horvitz1999principles,hearst1999mixed}, and multi-view visualizations (e.g.,~\cite{qu2017keeping,wang2000guidelines}), we compiled \todo{five} goals that informed \medley's design. We refined the user experience while iterating over early designs of the prototype.

\vspace{.5em}
\noindent\textbf{DG1. \change{Recommend a collection of views.} \cut{Treat collections as bags of options rather than dashboard recommendations.}}
\vidya{this design goal needs to be further unpacked. There is a precedence of `collection recommendations' from the music playlist and product domains. Attempted to elaborate...} 
Dashboards contain multiple views that contribute to an overall intent. We draw inspiration from the collection recommendation literature~\cite{hansen:2009,Golbeck2011AFF,singal:2021} wherein
items in a collection are complementary so that the relevance of each item is enhanced when combined with other items (e.g., Amazon’s ``Buy Together'' offers that provide one price for a bundle of related books). Users have the flexibility of picking the entire collection or a subset of items within the collection based on their interest. In the context of helping a user compose dashboards, the system should provide a collections of views such that the items in the collection are both relevant to the user and to the overall theme of the intent that the collection is recommended for. In other words, the recommended dashboard collections should act as a themed medley of views and widgets (thus inspiring the system name) and not as ``ready-to-use dashboard recommendations.'' In terms of system behavior, this translates to enabling authors to compose dashboards using a single recommended collection as a whole \emph{or} using views/widgets from multiple collections.

\vspace{.5em}
\vidya{I'm really having trouble understanding this goal.}
\noindent\textbf{DGx. Support and prioritize explicit user input.}
% Most participants were fine with this behavior and agreed that it provided ideas during a ``cold start'' scenario.
% However, two experts, in particular, were repelled by this system behavior and found it disruptive when they came to the system with specific attributes in mind and the system presented recommendations without taking their preference into account.
In some initial versions, we designed the prototype to exhibit more autonomous behavior.\vidya{what exactly was autonomous? Did a previous system ignore any form of user input, including which views were picked? That doesn't make much sense then.}
For instance, the system directly recommended collections upon data loading and over the course of a session, gave comparable weightage to explicit selections in the input panel and implicit information derived from views in the canvas.\vidya{what about explicit selections of the recommended views?}
However, interviewees (dashboard experts, in particular) felt that they were lacking control of the system's recommendations and it did not give enough preference to their domain knowledge.
This feedback, in combination with prior mixed-initiative visualization recommendation systems (e.g.,~\cite{key2012vizdeck,wongsuphasawat2017voyager,wu2021multivision}) translated to the goal that the system should allow users to explicitly specify their preferred attributes and intents \emph{at any point} in a session.
Furthermore, the system \emph{should prioritize explicit input} over any implicitly inferred information (e.g., attributes inferred from previously selected views) while generating recommendations.
% Furthermore, we initially viewed the recommended collections to be equivalent to dashboard recommendations (i.e., selecting a recommended collection would add all its views and widgets to a dashboard).

\vidya{feel like we also need to have a design goal on the recommendations themselves. For inferred attributes, we try to recommend views with low cardinality for instance. Do we allow for duplication of views across collections or are they mutually exclusive? How are widget recommendations surfaced? Do we account for the relevant vs. diversity tradeoff? What are some other aspects of the recommendation algorithm that would be relevant here - include picking up views and ordering as well. In summary, this goal should address minimizing and optimizing for a user being overwhelmed with all the options they get.}

\vspace{.5em}
\vidya{I think that this goal should be expanded to include text to explain system behavior in addition to summarizing the collections, given the complexity of the system. This should come last in the order of design goals as we first focus on the goals for system behavior.}
\noindent\textbf{DGx. Provide descriptive text to summarize collections and explain system behavior.}
Interpreting multi-view recommendations can be difficult since users not only need to inspect individual views but also their collective fit~\cite{wu2021multivision}.
While participants said that grouping views and widgets into collections was visually helpful, they further suggested adding brief textual descriptions to summarize the content within individual collections. \vidya{can we include details on adding text for filters in play w.r.t. widgets and interactive links?}
Providing feedback on initial versions of these descriptions, participants suggested using terms like ``measures'' (a common BI term used to refer to quantitative attributes) and ``dimensions'' (a common BI term used to refer to categorical and temporal attributes) so the text is more familiar for users of mainstream dashboard authoring tools like Tableau.
% Say something about using familiar BI terms like measure and dimensions.

\vspace{.5em}
\noindent\textbf{DGx. Support visual consistency in recommendations.}
% Current tools treat each view individually, but that leads to inconsistency during dashboard design...
% Since most current tools require users to author individual views and add them to a dashboard,
\vidya{we need to be careful about this design goal as Medley does not perform view snapping, alignment, or any other customization beyond just consistent color schemes. Rather, I'd generalize this to `Supporting visualization best practices' to include color encodings, chart type, and cardinality for recommending views.}
A key pain point mentioned during our interviews was around the customization required for achieving visual consistency across views in a dashboard.
Thus, similar to prior systems~\cite{wu2021multivision}, we noted that views recommended in \medley~should inherently incorporate multi-view design guidelines~\cite{qu2017keeping,wang2000guidelines} and be visually consistent across collections (e.g., a quantitative field is presented using the same color, the same color palette is used for categorical fields).\vidya{Is the visual consistency just around color? If so, I'd generalize this to include other best practices, like chart type (based on Show Me)}


\vspace{.5em}
\noindent\textbf{DGx. Provide support for interactions.}
\vidya{I don't understand what this sentence means when you say `varying levels of detail'. Thought Medley does not support LODs, but just filtering / highlighting.} Interaction between elements empowers a dashboard's users to ask and answer data questions at varying levels of overview and detail.
However, similar to prior studies (e.g.,~\cite{wu2021multivision}), our interviewees also mentioned that understanding the connectivity between dashboard elements and choosing the interaction technique (e.g., highlight versus filter) is a pain point with current tools.
This requirement motivated the need for a design goal of providing a lightweight interface for adding widgets and linking views during dashboard composition.

% \vspace{.5em}
% \noindent\textbf{DGx. Support customization.}

==> sections/archive/introduction-Mar20.tex <==
\firstsection{Introduction}
\maketitle

Visualization dashboards are commonly used across a range of applications that include finance, healthcare, sports, among many others. \vidya{feels like there is a missing transition sentence here. We should talk about why they are so prevalent first. We should also define what we mean by `views'} At a high-level, the process of creating dashboards can be broadly divided into two steps: 1) exploring the data to identify the views to include in a dashboard and 2) determining how these individual views are composited together in a visual layout with cross-view interaction.
Performing these steps can be tedious and challenging, however, requiring expertise with both data analysis and visualization design.
For the remainder of this paper, we use the term \textbf{\emph{dashboard}} to refer to a visual data representation structured as a tiled layout of views (numbers or canonical chart types such as bar charts, line charts, scatterplots, and maps) and filtering widgets (e.g., drop-downs, sliders).
\arjun{Need to loop in Few's definition (either here or in the related work): ``\textit{A dashboard is a visual display of the most important information needed \textbf{to achieve one or more objectives}; consolidated and arranged on a single screen so the information can be monitored at a glance.}"} \vidya{This should go in the intro where we introduce the term dashboard. The definition you currently have there is more about design and layout and less about the analytical objectives leading to its composition.}

Current visualization tools offer considerable support for creating individual views by recommending suitable visual encodings for a given set of data attributes (e.g.,~\cite{mackinlay1986automating,mackinlay2007show,wongsuphasawat2016towards,lin2020dziban}), recommending data attributes and views to consider (e.g.,~\cite{key2012vizdeck,vartak2015seedb,wongsuphasawat2015voyager,wongsuphasawat2017voyager}), and data facts or insights corresponding to individual views (e.g.,~\cite{demiralp2017foresight,cui2019datasite}). \vidya{I think they key takeaway we want to highlight here is that authoring a dashboard is often considered an `after thought' and not part of a user's analytical workflow. You have all the views suggested to you or you create the \emph{individual} views based on an analytical task, and then assemble them together. However, dashboards also tend to serve as analytical artifacts where the views and their interactions together support an analytical intent. This claim will need to be backed up though.}
However, existing systems offer limited support for users (i.e., dashboard authors) to discover and browse \emph{groups of views} that can be used to create a dashboard that helps convey a coherent message about the underlying data.
With this limited guidance for dashboard development, users are compelled to create a series of potentially interesting individual views, identify which views comply with their eventual dashboard's message, and then compose a dashboard with the relevant subset of views.
This sequential workflow results in dashboard creation becoming tedious and more of an afterthought than being an active part of the users' visual analysis process.

To make dashboard composition a more active process, we propose using the notion of \textbf{\emph{dashboard intents}}, or analytical goals that a dashboard's author wishes to enable/facilitate through a dashboard (e.g. ``Show year-over-year changes in the company's performance'').
We posit that visualization systems can leverage intents to provide recommendations that make the dashboard authoring process more accessible to users from different domains with varying levels of data and visual analysis experience.
Specifically, we discuss how intents can be used as facets or organizational anchors to recommend \emph{coherent sets of views and filtering widgets} (referred to hereon as \textbf{\emph{collections}}) that authors can browse to pick and choose their dashboard's content from.

To identify common analytical intents for authoring dashboards, we conducted a series of interviews with \vidya{how many and were they experts?} dashboard authors and surveyed \todo{XX} dashboards made with mainstream dashboard development tools like Tableau and Microsoft's Power BI.
From the interviews and survey results, we identified four high-level dashboard intents--- \emph{measure analysis}, \emph{change analysis}, \emph{category analysis}, and \emph{distribution analysis}, and collections corresponding to these intents. \vidya{we don't explain what these intents are}
Based on these dashboard intents and collections, we implemented \medley, a mixed-initiative interface that aids dashboard composition by recommending collections of views and widgets.
In addition to helping authors identify relevant views and widgets for their dashboards, \medley~also provides a lightweight direct manipulation-based interface for configuring interactions in the dashboard.
Based on a preliminary user study with \medley, we validate our premise that intent-oriented recommendations can support dashboard composition.
Finally, we consolidate our \vidya{not sure what `design experience' means here} design experience and study feedback to discuss promising avenues for future work including recommendation of dashboard layouts and designing natural language interfaces for dashboard authoring.

In summary, the primary contributions of our work include:
\vidya{need to include the survey and the dashboard intents as well}
\begin{itemize}
    \item We describe the design and implementation of \medley, a mixed-initiative interface that demonstrates the idea of recommending intent-oriented collections of views and widgets to aid dashboard development.
    \item We report findings from a preliminary user study with \medley~investigating how users with varying levels of dashboard design experience perceive and utilize the recommended collections.
    Participant feedback indicated that...
\end{itemize}

% \arjun{[MAYBE] Try writing an alternative/edited version of this intro that builds on the premise ``task-based viz rec has been successful for single-view recommendation, we wanted to try it for multi-view and dashboards..."}

==> sections/archive/recommendation-adi-Feb26.tex <==
\subsection{Collection Recommendation}
\begin{figure*}[t!]
    \centering
    \includegraphics[width=\textwidth,keepaspectratio]{figures/RecommendationDescription_V2.pdf}
    \caption{Steps involved in the recommendation of collections in~\medley. \aditeya{Add a separator between generation and ranking step.}}
    \label{fig:recommendationOverview}
\end{figure*}

\subsubsection{Collection Generation}
Collections in~\medley~require a set of attributes for generating the views and widgets. Input attributes for the system are either specified explicitly by the user. Otherwise,if the user does not specify the input, then \medley can infer attributes from the dashboard or by selecting potentially interesting attributes available in the dataset. In Fig.~\ref{fig:recommendationOverview} (1), shows that the user has selected ``Profit" attribute in the input panel of the system. However, to generate collections shown in Fig.~\ref{fig:recommendationOverview} (3) the system needs attributes besides ``Profit". Therefore in this case, the system infers the remaining attributes from two sources. First the system realizes that the user has already added ``Sales datasummary" and a ``Sales by State" chart to the dashboard. Therefore based on this state of the dashboard, the system infers that the user is probably interested in the ``Sales" and ``State" attributes. Besides, ``Profit", ``Sales" and ``State" the system needs additional attributes to create the final set of views and widgets. So at this point, when the system has no further indication of what attributes the user is interested in but it still need attributes to populate the collections then it is uses the data intersestingness measure to infer remaining attributes from the dataset. All the inferred attributes alongwith selected attributes are shown in Fig.~\ref{fig:recommendationOverview} (step~2).

\textbf{Data Interestingness:} \aditeya{People maybe interested in details of data interestingness so we should explain it briefly here. Talk about the design goal related to data interstingness}

After \medley~identifies or infers all the attributes, the next step in recommendation pipeline is generation of the collection. Views and widgets are pre-configured into the system in forms of collection templates \aditeya{this may need to be talked in the system section}. Therefore in this step, \medley~reads the data requirement for each view from the template and then assigns it the appropriate attribute. For example in Fig.~\ref{fig:recommendationOverview} (3), the first chart in the first collection at an abstract level the view needs a quantitative and temporal attribute to calculate the change and a geo attribute to show changes. Therefore \medley~looks up in the list of attributes in Fig.~\ref{fig:recommendationOverview} (2) and assigns the view a quantitative attribute ``Profit", a temporal attribute ``date" and a geo attribute ``state". The attributes identified and used for collection generation also have an inherent ordering. When generating collections, \medley~gives highest priority to attributes that were selected explicitly by the user in the input panel. Next level priority is given to attributes inferred from dashboard. The last level of priority is given to attributes selected using the data interestingness score. Between dashboard and data interestingness attribute, we chose to give dashboard attributes more priority because they indirectly capture user's interest. Whereas data interestingness attributes may be very relevant from statistical aspect, but the attribute may not be of much interest to the user. In order to understand the priority order, let us analyze collection 2 in Fig.~\ref{fig:recommendationOverview} (3). In the collection, we can notice that the first chart is a barchart that summarizes change across all years for ``Profit" attribute and the second chart shows ``Sales" attribute. This happens because system gives ``Profit" attribute priority.


\aditeya{We support this partially, but the code can be extended easily to handle this case}
A special case for collection generation is when the input dataset does not have sufficient attributes for the system to infer and populate collections. To handle this case, ~\medley~removes views from collections or the entire collection. \aditeya{Give an example of the change template that they will be removed if there is no time attributes and also remove time views from other collections}


\subsubsection{Ranking of Collections and Views}

\medley's~ranking algorithm reveals relevant collections to the user based on their data and intent requirements. If the user directly specifies an intent to the system, then ~\medley~only displays collections that are relevant for the intent. For example in Fig.~\ref{fig:recommendationOverview} (1) the user has explicitly selected the ``Change Analysis" intent so the system recommends collections that are relevant to change. However, for change the system has two relevant collection options. In this case, the system ranks the collections to bring to the top more relevant ones.

\vspace{.5em}
\textbf{Collection Ranking With Attributes from Input Panel:} When the user specifies the attributes of interest in the input panel, then the system uses these attributes to rank collections. In Fig.~\ref{fig:recommendationOverview}, the user has specified that they are interested in analyzing the ``Profit" attribute. Moreover, they have selected the ``Change Analysis" intent. Therefore, \medley~needs to determine the ranking between change collections ``CH1" and ``CH2" from Table~\ref{tbl:collection}. \medley~uses the Jaccard Similarity Index\aditeya{CITE} for calculation of similarity between the user input and the required attributes for the collection. Jaccard Similarity calculates a ratio of shared members across two sets. \medley~uses this score to calculate similarity between user input and the required attributes for collections listed in Table~\ref{tbl:collection} (Attributes column). \medley~does not consider the exact attribute name but instead uses the data type of the attribute for the calculation of similarity. For Fig.~\ref{fig:recommendationOverview} (1), the input set IP:\{q1\} and the required attribute set for CH1:\{q1,t1\} and for CH2:\{q1,q2,t1\}. The Jaccard Similarity score for \textbf{IP vs. CH1 is 0.5}, whereas the \textbf{IP vs. CH2 is 0.3}. Therefore, in Fig.~\ref{fig:recommendationOverview} (3) collection CH1 is recommended over CH2.

\vspace{.5em}
\textbf{Collection Ranking With Attributes Inferred from Dashboard:} If the user does not choose input attributes explicitly in the input panel but adds views to the dashboard. In that case, \medley~uses the attributes inferred from the dashboard to rank collections. In Fig.~\ref{fig:recommendationOverview} (2),since the user has selected an attribute from the input panel (``Profit"), the attributes inferred from dashboard (``Sales" and ``State") are not used for recommendation. The ranking technique is the same as described previously. In this case, \medley~uses Jaccard Similarity for ranking collections.

\vspace{.5em}
\textbf{Collection Ranking Without Input Attributes:} To support use-cases, where the user does not have any specific intent or attributes in their mind. That means, they are primarily looking to explore the collections in the system. In these situations, \medley~orders collections to communicate the wide range of options users have to author their dashboards. Therefore, in this case, \medley~shows one collection from each intent first and then repeats it in the same pattern. An example of this default recommendation is shown in \aditeya{REFER TO SCENARIO FIG} option 1. As shown in that figure, the collections shown are distribution, measure, category and change.

\vspace{.5em}
\textbf{Ranking Views within Collections:} In addition to the collections, the views within the collections are also ranked in \medley. To rank views within the collections, \medley~uses the same technique of ranking collections, where a similarity score is computed between the explicit input and inputs inferred from dashboard and attributes required by each view. For example, in Fig.~\ref{fig:recommendationOverview} explicit and dashboard input include three attributes: ``Profit", ``Sales" and ``State". Therefore the abstract input representation in this case becomes \{q1,q2,t1\}. Based on the abstract input, the map view in Fig.~\ref{fig:recommendationOverview} (3) first collection is the view that has the highest similarity to the input requirement, therefore it is placed first in the chart. Other views in the collection are then ordered based on their similarity score with the input.
There is however one caveat to the view ranking. If a view is added to the dashboard that view is sent to the bottom of the list. Reordering of view along with a visual fading out ensures that the users are aware that they already have this view in the template. \aditeya{REF to TEASER}





% \textbf{Discussion Points}

% Nested levels of Recommendation
% 1. Collection Recommendation
%     1. 1 View Recommendation
%     1.2 Widget Recommendation

% Recommendation Flows:
% 1. Default Recommendation
% 2.Recommendation through the input attributes
% 3. Recommendation through addition of views to the dashboard (with no attributes)
% 4. Recommendation when input attributes are provided and views are added to dashboard

% Recommendation Factors:
% 1. Intent Similarity with Collections
% 2. View Similarity within Collections based on attributes selected or in dashboard
% 3. Coverage: when views are added to the dashboard
% 4. Diversity: when there is no input from the user

% Collection Generation: available attributes and generation of the ranking

% Collection Ranking: Percentage similarity. If user selects 1q and 1t, then the similarity score is computed with all collections. Similarity score is matching percentage between available and focus attributes. In this case the ``YoY" will have 100 similarity.

% View Ranking within Collection


% Intent Faceting (This should be talked very briefly in the end)




==> sections/archive/scenario-Feb21.tex <==
\section{Usage Scenario}
\vidya{the way this scenario section is currently written, it references the design goals. Based on our discussion, if this precedes the design goals, it needs to be a higher-level and reference the scenario in the Design Goals section.}

We describe two exemplary usage scenarios to illustrate how the system supports different dashboard composition workflows (the scenarios are also presented in a supplementary video).
For both scenarios, we use a dataset that represents sales for a fictitious company \vidya{Hmmm can we not use Superstore for the scenario? It's rather overused and is very Tableau}``Superstore'' located in the USA\footnote{The dataset is provided in the supplementary materials and is a subset of the popular Superstore dataset that appears as one of the sample datasets in Tableau.}.
Each row in the dataset is a sale and there are \todo{XX} columns including \todo{XX} quantitative attributes (e.g., {\small{\faHashtag}}~\textit{Sales}, {\small{\faHashtag}}~\textit{Profit}), \todo{XX} categorical attributes (e.g., {\small{\faFont}}~\textit{Category}, {\small{\faFont}}~\textit{Segment}), one geographic attribute ({\small{\faGlobe}}~\textit{State}), and \todo{a} temporal attribute ({\small{\faCalendar}}~\textit{ShipDate}).
For consistency, we use this dataset as an example throughout this section.

\subsubsection{Composing Dashboards based on a priori Goals}

\begin{figure}[t!]
    \centering
    \includegraphics[width=\linewidth]{figures/scenario-1-1.pdf}
    \caption{Scenes from the first usage scenario. (A) Default recommendations when no attributes or intents are selected. (B) Recommendations when the \textit{Change Analysis} intent is selected in the input panel. (C) Recommendations when \textit{Change Analysis} and \textit{Profit} is selected in the input panel with two views already added to the dashboard canvas.}
    \label{fig:scenario-1}
\end{figure}

\vidya{I'm tempted to put in a name from https://time.com/100-women-of-the-year/ :)}
Imagine Sarah, an operations reporting analyst who designs dashboards for the Superstore company's executives.
As part of the annual review meeting, Sarah needs to compose a dashboard that can help ``\textit{understand the company's performance over time}''.
With this goal in mind, Sarah loads the dataset into \medley.

To begin, the system gives her the choice of selecting \vidya{why and /or? the system provides both.} attributes and/or intents she is interested in or \vidya{I don't understand this following phrase and how it's different from intents} directly view some recommended collections (\todo{DGx}).
As she only has a high-level goal in mind with no specific idea of what she would like to include in her dashboard, Sarah requests to see the default recommendations in \medley.
In response, \medley~recommends a list of collections for Sarah to consider (Figure~\ref{fig:scenario-1}A).
Each collection maps to one of the four intents described in Section~\ref{}.
As Sarah has not yet indicated interest in any specific attributes or intents, \medley~orders its recommendations to present one sample collection for each intent.
For example, in Figure~\ref{fig:scenario-1}A, the first collection maps to the \textit{Distribution Analysis} intent and presents univariate summaries of the different attribute.
The second \textit{Measure Analysis} collection presents views and widgets that can help compose a dashboard to analyze a single measure (\textit{Sales}) across different dimensions (e.g., \textit{State}, \textit{Segment}, \textit{ShipDate}) (\todo{DGx}, the system provides a description of the collection to Sarah).
Skimming through the recommended collections, Sarah finds the fourth \textit{Change Analysis}-oriented recommendation of the collection summarizing ``Year-over-year (YoY) change in Sales'' interesting as this aligns with her dashboard design goal.
To filter the recommendations and focus on collections mapping to the \textit{Change Analysis} intent, Sarah selects the intent in left panel.

\medley~now updates its recommendations to only show the two collections that map to \textit{Change Analysis} (Figure~\ref{fig:scenario-1}B).
While the first collection presents views that focus on one year at a time and show differences relative to the previous year for a single attribute (\textit{Sales}), the second collection displays data for all years with views explicitly encoding yearly changes for two attributes (\textit{Sales} and \textit{Profit}).
At this point, Sarah can add one or both collections to the dashboard canvas as-is ({\small{\faPlus}}), or pick and choose specific content from individual collections (\todo{DGx}).
From the second collection, Sarah likes the idea of using multiple measures in her dashboard, but wants to use the views of the first collection to analyze change one year at a time.
Correspondingly, Sarah starts by adding two views (the bar chart showing YoY change for \textit{Sales} by \textit{Category} and the choropleth map) from the first collection to the dashboard canvas.
Next, to see similar YoY change views for \textit{Profit}, Sarah selects the \textit{Profit} attribute in the input panel.
In response, \medley~updates its recommendations to switch the focus of the first collection from \textit{Sales} to \textit{Profit} (Figure~\ref{fig:scenario-1}C). Considering the two views already in the canvas, the system also ranks the views within the first collection such that the bar chart and map are shown first.
Sarah adds the two views to the canvas, which now has four views (two bar charts and two maps corresponding to \textit{Sales} and \textit{Profit}, respectively).
Sarah also notices that \medley~has suggested a year picker widget along with the first collection and adds this to her canvas as it will enable her dashboard viewers to select specific years to focus on.

Looking at the current canvas, Sarah feels she has a good set of views to support an analysis of the YoY changes but lacks an overview summarizing the total sales and profit for an year.
With this thought in mind, Sarah deselects the \textit{Change Analysis} intent from the left panel and gets a new set of collection recommendations from \medley (Figure~\ref{fig:interface}B).
Considering the active attribute in the left panel (\textit{Profit}) and views in the canvas, the system ranks its recommendations such that a \textit{Change Analysis} collection is shown first followed by \textit{Measure Analysis} collections.
Looking at the fourth collection, Sarah sees a recommended view showing the numeric summary of total \textit{Profit} and \textit{Sales}, adds it to the canvas, and edits view sizes and layout to make the dashboard more presentable (\todo{DGx}) (Figure~\ref{fig:interface}B,C).

\vidya{this para below can be tightened.}
As Sarah was adding views and widgets to the canvas, \medley~also implicitly configured interactions between the dashboard elements (i.e., clicking a view to filter other views, updating all views when the year filter widget is toggled \vidya{toggled or filtered to a year?}).
Testing the \vidya{are we using cross-view or coordinated views?} cross-view interactions, Sarah notices that \medley~has configured the interactions such that when she clicks a state on one of the choropleth maps, the non-matching states in the other map fade out but retain their color akin to a brush- or highlight-style interaction.
However, because of the continuous red-blue color scale used for the map, she feels it would be difficult for her viewers to read the values correctly and detect which state is highlighted.
To update this interaction behavior, Sarah clicks the {\small{\faLink}} icon on the \textit{Profit} map on the left and \medley~shows her the connections between the map and the other views through links overlaid on the canvas itself (\todo{DGx}) (Figure~\ref{fig:interface}C).
She sees that the map is linked to the \textit{Sales} map on the right via a highlight link ({\small{\faMagic}}) and changes this to a filter link ({\small{\faFilter}}), and repeats this process for the \textit{Sales} map on the right.
Now when Sarah clicks on a state in the map, only that state is displayed in the other map, making it easier to read the mark's value.
Satisfied with the dashboard she put together, she downloads the dashboard to share with her team.

\vidya{I prefer the first scenario as it illustrates intent-based recommendations more effectively than the attribute-based on that you discuss below.}
\subsubsection{Ad hoc Dashboard Composition}

% The above scenario illustrated a case where the author had a very specific dashboard goal in mind (``Showing year-over-year changes").
As a second scenario, Joe is an analyst who has newly joined the \vidya{again, prefer an alternative name} Superstore company.
Joe wants to compose a dashboard that can help him gain a general understanding of the company's sales.
Note that unlike the first scenario, in this case, the user has an attribute in mind (\textit{Sales}) but no specific goal or intent they are trying to create a dashboard for (e.g., ``\textit{understand the company's performance over time}" in the first scenario).

Joe loads the data into \medley~and given his interest in analyzing the company's sales, selects the \textit{Sales} attribute from the input panel.
In response, \medley~recommends a list of collections, ranking \textit{Measure Analysis} collections that focus on \textit{Sales} as a primary measure higher than other collections (Figure~\ref{fig:scenario-2}A).
Skimming through the collections and their underlying themes, Joe narrows in on the first collection that focuses on the ``\textit{Analysis of \textit{Sales} across dimensions}." To summarize total \textit{Sales}, Joe adds the data summary view from the first collection to his dashboard canvas.
Furthermore, to see the breakdown of \textit{Sales} by \textit{State}, Joe also adds the choropleth map to the canvas.

Inspecting other views in the first collection, Joe observes a difference in \textit{Sales} across \textit{Segment}, noting that sales for the `Consumer' segment are significantly higher. To further explore this variation in \textit{Sales}, he selects the \textit{Segment} attribute in the input panel, resulting in \medley~updating its recommendations (Figure~\ref{fig:scenario-2}B).
Joe notices that the system now presents a new \textit{Category Analysis} collection that focuses on the theme of ``\textit{Summary of \textit{Sales} by \textit{Segment}}" as one of its top recommendations (Figure~\ref{fig:scenario-2}B, right).
Inspecting the new collection, Joe adds three views (a bar chart of \textit{Sales} by \textit{Segment}, and two grouped bar charts visualizing \textit{Sales} by \textit{Category} and \textit{Sales} by \textit{ShipMode}, both broken down by \textit{Segment}) that can help him understand differences in \textit{Sales} between segments to the dashboard canvas. Joe also notices that \medley~suggests adding a range slider for \textit{ShipDate} as one of the widgets to complement the views. Realizing that the slider would allow him to look at the sales over different periods of time, Joe adds the widget to the canvas.

\begin{figure}[t!]
    \centering
    \includegraphics[width=\linewidth]{figures/scenario-2-1.pdf}
    \caption{Scenes from the second usage scenario. (A) Recommended collections when the \textit{Sales} attribute is selected. (B) Updated recommendations when \textit{Segment} is selected in addition to \textit{Sales}. (C) Final dashboard composed using a mix of views and widgets from the two collections shown in (B).}
    \label{fig:scenario-2}
\end{figure}

With five views and a widget added to the canvas (all interactively linked by default), Joe now has a dashboard that enables him to get an overview of the company's sales, as well as dive into specific data subsets to understand the trend and distribution of sales for different product segments.
For instance, by clicking on segments in the \textit{Sales} by \textit{Segment} bar chart and seeing the changes in the other charts, Joe make observations such as the sales for `Consumer' products could be even higher if the company expanded into the states of Maine and Wyoming, the product categories `Furniture' and `Office Supplies' are contributing relatively lower sales than `Technology' for the `Home Office' segment, and so on.
Joe updates the dashboard's layout to make it more presentable, and shares the dashboard and his findings with his colleagues for further discussion during their next meeting (Figure~\ref{fig:scenario-2}C).

\arjun{May need to drop the second scenario to buy space for subsequent sections and also make figures bigger.}

==> sections/archive/xx-intent.tex <==
\begin{figure}[t!]
    \centering
    \includegraphics[width=\columnwidth,keepaspectratio]{figures/IntentDashboardV2.pdf}
    \caption{High-level dashboard intents and their examples. \textbf{A:} Shows analysis of the measure ``Sales" across ``Region",``Employee" and ``Year" dimensions\aditeya{CITE}.\textbf{ B:} Shows ``YoY Sales" change by ``Region" and ``Time".\aditeya{CITE} \textbf{C:} Shows the distribution of percentages and counts of of categorical variable ``Student Type" across other dimensions such as ``Time", ``Degree Program", and ``PhD Program"\aditeya{CITE}. \textit{Titles are modified to enhance readability.}}
    \label{fig:intentsdashboard}
\end{figure}

\section{Identifying Dashboard Intents}

\aditeya{This section is written with an assumption that intents and collections have been previously introduced to the reader}

\vidya{this para (or at least a portion of it) should come after you talk about the survey and identify the design goals for Medley. Also, until now there is not mention of intents for even charts. I know that Arjun mentioned that he wants to bring it later during the scenario, but it seems odd not to talk about prior work around analytical intent and why we decided to go into a survey. Your sentence below in this para is not sufficient to motivate it.}
\medley~recommends relevant views and widgets based on the high-level dashboard authoring intent of the user. However, existing work in visualization literature does not provide sufficient guidance on ``What are the different high-level intents of the user when they author dashboards?" Therefore, we introduce and discuss high-level intents for dashboard authoring in this section.

To better understand what high-level intents authors have in mind when composing dashboards, we conducted a survey of 300 public dashboards from Tableau~\cite{tableau2022} and Microsoft's  Power BI~\cite{mspbi2022}. We chose Tableau and Power BI because they tend to be widely used tools for authoring dashboards. Moreover, their public platforms include a wide range of dashboards that users create. To search for candidate dashboards, we reviewed both curated galleries and also used the search functionality on Tableau Public~\cite{tableaupublic2021link} and Microsoft Power BI Gallery~\cite{microsoftpbi2021link}. Combined Tableau Public and Microsoft's Power BI contain over several thousand dashboards. It was beyond the scope of this work to analyze all the dashboards. Therefore, the survey focused on dashboards that have two or more basic visualizations that are currently supported by Tableau and Power BI. Fig.~\ref{fig:intentsdashboard} includes three example dashboards included in the survey. The survey excludes dashboards that appeared as infographics or the dashboards had complex charts. The "Visual History of F1 Tableau" by James Smith~\cite{smith2019dashboard} is an example of dashboard that was not included from the survey because of the infographic design. The dashboards from the survey are provided in the supplemental material.

To identify the dashboard intents, each author categorized dashboards into groups based on the visualizations, widgets, interaction between views and widgets, title, and other meta-data such as textual description. For each group, authors inductively derived a theme that encapsulated the high-level goal of the dashboard. For example, Fig.~\ref{fig:intentsdashboard} \textbf{A} focuses on the analysis of ``Sales" across other dimensions such as ``Region",``Employee", therefore the dashboard was marked as a ``Measure Analysis" dashboard. Whereas in Fig.~\ref{fig:intentsdashboard} \textbf{B}, the dashboard shows change in sales, more specifically ``Year over Year (YoY)" change, therefore the dashboard was categorized as ``Change Analysis". After the individual tagging step, all the authors discussed their tagging until they reached a consensus. Based on the qualitative coding and agreement, four distinct categories of high-level intents emerged from the survey: 
\begin{itemize}
  \item \textit{Measure Analysis}: Supporting the analysis of one or more measure fields (Fig.~\ref{fig:intentsdashboard} \textbf{A}, ``Analyzing Sales").
  \item \textit{Change Analysis}: Presenting the change in measure over time (Fig.~\ref{fig:intentsdashboard} \textbf{B}, ``Displaying YoY change in Sales").
  \item \textit{Category Analysis}: Analyzing a dataset with a focus on one or more categorical variables (Fig.~\ref{fig:intentsdashboard} \textbf{C}, ``Visualizing Student Type (International vs. Domestic) across different academic programs").
  \item \textit{Distribution Analysis}: Summarizing the number/count of items with respect to different categorical and quantitative attributes in the dataset (e.g. ``Showing the number of employees in different departments, salary brackets, etc.").
\end{itemize}
After identifying the high-level intents, we validated them through formative interviews with dashboard experts. These experts have years of experience creating and designing dashboards for Tableau's customers or internal teams. Most experts agreed that the high-level intent categories exhaustively cover most of their dashboard authoring use-cases. The interviews reassured us that the intents we identified through the survey would help develop \medley. Intent tagging of dashboards is available in the Supplemental Material.

High-level intents are helpful for a broad classification of dashboard intents. However, for creating recommendations in \medley~we realized that we need to break each high-level intent to a \textit{sub-intent} that can describe a dashboard in more detail. For example,  when we analyzed the dashboards tagged with measure analysis intent, we noticed dashboards with a few different patterns. A typical pattern was ``Comparing two or more measures". In these dashboards, authors focus on comparing measures available in the dataset, such as ``Sales" and ``Profit" . Another common sub-intent for measure analysis is the analysis of ``Top measure values". Top or bottom analysis is used when the user wants to look at top values for a high-cardinality variable. An example of top or bottom analysis dashboard can be an analysis of ``Sales" by ``Employees" or ``Products".

\aditeya{Fig XXX} lists the sub-intents corresponding to the intents and includes a reference to a sample dashboard corresponding to the sub-intent. In \medley~sub-intents play a crucial role because they map directly to a collection of visualizations and widgets as shown in FIG XXX. A collection in \medley~consists of visualizations and widgets that are carefully curated to assist users in authoring a dashboard. To curate the collections, we surveyed the common visualizations and widgets used by dashboards in each category of sub-intent and used that information to create a sample collection. Please refer to the Supplemental Materials for more details on the collection curation from the surveyed dashboards.

% However, while analyzing the dashboards we also noticed that that many times dashboards can fall into more than one intent identified in \medley. Specifically to handle this situation, \medley supports picking views and widgets from multiple collections to author the dashboards. We expand on the pick and choose feature of \medley in \aditeya{ DESIGN CONSIDERATIONS SECTION} and \aditeya{SYSTEM SECTION} of the paper.

% \aditeya{Talk about LinPack as additional motivation for the idea of using templates/collections. --- IMO this should be introduced and discussed in the related works section and we can briefly talk about it in this section}

% \input{tables/intents}

\begin{figure*}[t!]
    \centering
    \includegraphics[width=\textwidth,keepaspectratio]{figures/Intent_Themes_Collections_V2.pdf}
    \caption{Summary of dashboard intents with corresponding themes. Each theme includes a link to an example dashboard, focus attributes and a description of the recommended collection.}
    \label{fig:collection}
\end{figure*}

==> tables/intents.tex <==
\begin{table*}[t!]
        \caption{Intents, sub-intents, collections}
\begin{center}
{
    \begin{tabular}{P{3cm} P{4cm} P{2cm}  P{8cm}} 
         \textbf{Intent}  & \textbf{Sub-Intent} & \textbf{Attributes Req.} & 
         \textbf{Collection (Views + Widgets)}  \\ 
       \hline
       \\
Measure Analysis & Single Measure Summary & 1q & \begin{minipage}{.3\textwidth}
      \includegraphics[width=8cm, height=1.5cm]{figures/collections/M1_C1.pdf}
    \end{minipage} \\
Measure Analysis & Top N Analysis   & 1q & \begin{minipage}{.3\textwidth}
      \includegraphics[width=8cm, height=1.5cm]{figures/collections/M1_C1.pdf}
    \end{minipage}  \\
Measure Analysis & Measure Comparison\aditeya{CITE}   & 2q & \begin{minipage}{.3\textwidth}
      \includegraphics[width=8cm, height=1cm]{figures/IntentDashboard.pdf}
    \end{minipage}  \\
Measure Analysis & Measure Comparison\aditeya{CITE}   & 1t,1q & \begin{minipage}{.3\textwidth}
      \includegraphics[width=8cm, height=1cm]{figures/IntentDashboard.pdf}
    \end{minipage}  \\
\hline
Change Analysis & YoY Change\aditeya{CITE}   & 3q+ & \begin{minipage}{.3\textwidth}
      \includegraphics[width=8cm, height=1cm]{figures/IntentDashboard.pdf}
    \end{minipage}  \\
Change Analysis & Change Overview\aditeya{CITE}   & 1q+, & \begin{minipage}{.3\textwidth}
      \includegraphics[width=8cm, height=1cm]{figures/IntentDashboard.pdf}
    \end{minipage}  \\
\hline
Category Analysis & YoY Change\aditeya{CITE}   & 3q+ & \begin{minipage}{.3\textwidth}
      \includegraphics[width=8cm, height=1cm]{figures/IntentDashboard.pdf}
    \end{minipage}  \\
Category Analysis & Change Overview\aditeya{CITE}   & 1q+, & \begin{minipage}{.3\textwidth}
      \includegraphics[width=8cm, height=1cm]{figures/IntentDashboard.pdf}
    \end{minipage}  \\
    Category Analysis & YoY Change\aditeya{CITE}   & 3q+ & \begin{minipage}{.3\textwidth}
      \includegraphics[width=8cm, height=1cm]{figures/IntentDashboard.pdf}
    \end{minipage}  \\
    \hline
    Distribution Analysis & -\aditeya{CITE}   & 3q+ & \begin{minipage}{.3\textwidth}
      \includegraphics[width=8cm, height=1cm]{figures/IntentDashboard.pdf}
    \end{minipage}  \\
    \end{tabular}
    }
    \label{tab:surveyedpapers}   
\end{center}
\end{table*}
